Covariant spatio-temporal receptive fields for spiking neural networks

Biological nervous systems constitute important sources of inspiration towards computers that are faster, cheaper, and more energy efficient. Neuromorphic disciplines view the brain as a coevolved system, simultaneously optimizing the hardware and the algorithms running on it. There are clear efficiency gains when bringing the computations into a physical substrate, but we presently lack theories to guide efficient implementations. Here, we present a principled computational model for neuromorphic systems in terms of spatio-temporal receptive fields, based on affine Gaussian kernels over space and leaky-integrator and leaky integrate-and-fire models over time. Our theory is provably covariant to spatial affine and temporal scaling transformations, and with close similarities to the visual processing in mammalian brains. We use these spatio-temporal receptive fields as a prior in an event-based vision task, and show that this improves the training of spiking networks, which otherwise is known as problematic for event-based vision. This work combines efforts within scale-space theory and computational neuroscience to identify theoretically well-founded ways to process spatio-temporal signals in neuromorphic systems. Our contributions are immediately relevant for signal processing and event-based vision, and can be extended to other processing tasks over space and time, such as memory and control.

==> sections_rebuttal/methods_old.tex <==
All code and data required to reproduce the results in this paper can be found at \url{https://github.com/jegp/nrf}.

\subsection*{Biological neuron models} \label{sec:compneuro}
We use the leaky integrate-and-fire formalization from Lapicque \cite{Blair_1932, Abbott_1999}, stating that a neuron voltage potential $u$ evolves over time, according to its time constant, $\mu$, and some input current $I$

\begin{equation} \label{eq:li_dot}
  \mu\, \dot{u} = -u + I
\end{equation}
with a threshold function parameterized by $\theta_{threshold}$

\begin{equation} \label{eq:heaviside}
  z(t) = \begin{cases}
    1 & u >= \theta_{threshold} \\
    0 & u < \theta_{threshold}
  \end{cases}
\end{equation}
and a jump condition for the membrane potential, which resets to $\theta_{reset}$ when the threshold is crossed

\begin{equation} \label{eq:reset_instant}
  u(t) = \begin{cases}
    \theta_{reset} & z(t) = 1 \\
    u(t)           & z(t) < 1
  \end{cases}
\end{equation}
The \textit{firing} part of the leaky integrate-and-fire model implies that neurons are coupled solely at discrete events, known as \textit{spikes}.
%  nervous tissue, local and analog processes communicate via digital, discrete, signals.
% It is still unknown exactly why biology converged to this mixed analog and digital representation, although it is clear that digital signals avoid temporal dispersion across long distances, and convincing arguments have been made towards the computational efficiency of mixed-signal paradigms \cite{Sarpeshkar_1998}.
% However, some nervous systems, such as in the Caenorhabditis Elegans nematode, avoid the threshold altogether and communicate purely based on graded potentials induced by the leaky integrators as in equation \eqref{eq:li_dot}.

\subsection*{Spike response model} \label{sec:srm}
\begin{figure}
  \includegraphics[width=0.9\textwidth]{figures/srm.pdf}
  \caption{
    The spike response model recasts the leaky integrate-and-fire model as a composition of three filters: a membrane filter in blue ($\kappa$), a threshold filter in red ($H$), and a reset filter in green ($\eta$).
    The graphs inside the filters depict their respective outputs over time using the kernels in \eqref{eq:srm}, given some input signal, $I$.
  }
  \label{fig:srm}
\end{figure}

Gerstner et al. presented a generalized description of arbitrary neuron models as a compositions of filters, dubbed the Spike Response Model \cite{Gerstner_Kistler_Naud_Paninski_2014}.
The integration of the membrane voltage with the Spike Response Model can be described as a combination of a membrane reset filter ($\eta'$) following a spike generating function ($\Gamma$), and a subthreshold integration term ($\kappa$) given some input current ($I$) (see Figure 2 in the Supplementary Material):

\begin{equation} \label{eq:srm}
  u(t) = \int_0^{\infty} \eta'(s)\, \Gamma(t - s) + \kappa(s)\,I(t - s)ds
\end{equation}

% According to power law \cite{Pozzorini_Naud_Mensi_Gerstner_2013}

% The leaky integrate-and-fire model above approximates the laws governing the movement of electrons in circuits and, by extension, the laws of diffusion.
% The simpler first-order integrator in equation \ref{eq:li_dot} appears repeatedly in the study of diffusion and heat exchange \cite{Berg_1993} (see Appendix \ref{scale_diffusion}).
% More intricate, and more accurate, models of ion channels and charge travelling down axons or dendritic trees were derived later in the Goldman equation \cite{Goldman_1943} and the work by Hudgkin \cite{Hodgkin_Rushton_Adrian_1946} and Huxley \cite{Hodgkin_Huxley_1952}.

This formulation generalizes to numerous neuron models, but we will restrict ourselves to the LIF equations, which can be viewed as a composition of three filters: a membrane filter ($\kappa$), a threshold filter ($H$), and a membrane reset filter ($\eta'$) shown in Figure \ref{fig:srm}.
The spike response model defines neuron models as a composition of parametric functions (filters) of time \cite{Gerstner_Kistler_Naud_Paninski_2014}.
The membrane filter and membrane reset filter describes the subthreshold dynamics as follows:

\begin{equation} \label{eq:srm}
  u(t) = \int_0^\infty \eta'(s)\,\Gamma(t - s) + \kappa(s)\,I(t - s)\,ds
\end{equation}
The reset filter, $\eta'$, can be understood as the resetting mechanism of the neuron, that is, the function controlling the subthreshold behaviour immediately after a spike.
This contrasts the LIF formalism from equation \eqref{eq:reset} because the resetting mechanism is now a function of time instead of a constant.

Since the resetting mechanism depends entirely on the time of the threshold activations, we can recast it to a function of time ($t$), where $t_f$ denotes the time of the previous spike

\begin{equation} \label{eq:eta_spike}
  u(t) = \eta(t - t_f) + \int_0^\infty \kappa(s)I(t - s)ds
\end{equation}
Following \cite[eq. 6.33]{Gerstner_Kistler_Naud_Paninski_2014} we define $\eta$ more concretely as a linearized reset mechanism for the LIF model
\begin{align}  \label{eq:srm_eta}
  \eta(t - t_f; \mu_r) = -\theta_{thr}\ e^{-(t - t_f)/\mu_r}
\end{align}
The above equation illustrates how the ``after-spike effect'' decays at a rate determined by $\mu_r$.
Initially, the kernel corresponds to the \textit{negative} value of $\theta_{thr}$ at the time of the spike, effectively resetting the membrane potential by $\theta_{thr}$.
In the LIF model, the reset is instantaneous, which we observe when $\mu_r \to 0$.
This is visualized in Figure \ref{fig:srm} where the set of filters correspond to the subthreshold mechanism in equation \eqref{eq:li_2} (which we know to be scale covariant from equations \eqref{eq:trunc_exp_temporal_covariance}), the Heaviside threshold in equation \eqref{eq:heaviside}, and the reset mechanism in equation \eqref{eq:srm_eta}.

We arrive at the following expression for the subthreshold voltage dynamics of the LIF model:

\begin{equation} \label{eq:srm_base}
  z(t) = -\theta_{thr}\ e^{-(t - t_f)/\mu_r} + \int_0^\infty \kappa(s)\,I(t - s)\,ds
\end{equation}


\subsection*{Event-based vision} \label{sec:ebv}
\begin{figure}
  \includegraphics[width=\textwidth]{figures/img_cat.png}
  \caption{
    \textbf{Left}:
    Conventional cameras emit dense frames at discrete time intervals, here using a $32 \times 32$ image from the CIFAR10 dataset.
    \textbf{Right}: event cameras emit point clouds over space and time, here showing an arm moving in circles from the DVS gesture dataset \cite{Amir_2017}.
    Red and blue events indicate positive and negative polarity changes, respectively.
  }
  \label{fig:event_image}
\end{figure}
Biological vision sensors rely on photoreceptors to transduce light into electric potentials, to be processed by downstream neurons.
Similar to their natural counterparts, silicon retinas rely on \textit{logarithmic changes} of luminosity over time, providing an astonishing dynamical range of more than 120dB.
The analog nature of the photoreceptors yields favourable energy profiles, but also frees individual pixels to react to luminosity changes independently.
Consequently, event cameras produce sparse temporal streams of discrete polarity changes with a temporal resolution of the order of microseconds \cite{Lichtsteiner_Posch_Delbruck_2008}.
Figure \ref{fig:event_image} contrasts this with conventional, dense video frames.

Mathematically, we can consider event camera data as tuples of four numbers indicating time ($t$), x-y coordinates in the camera plane, and positive or negative polarity ($p$):

\begin{equation}
  ev_i = \{t_i, x_i, y_i, p_i \},\;\;\;\;\; i \in \mathbb{N}
\end{equation}

\subsubsection{Spatio-temporal event surfaces} \label{sec:ebv:surfaces}
The structure and shape of the event ``point cloud'' seen in Figure \ref{fig:event_image} are known to be significant for event-based vision algorithms \cite{Gallego2019,Tayarani_2021}.
\cite{Lagorce_Orchard_Galluppi_Shi_Benosman_2017} studied an extended form of point clouds, where events are ``stretched out'' in the temporal domain using a leaky integrator similar to \eqref{eq:li_dot}.
Concretely, incoming positive or negative events in camera coordinates

\begin{equation}
  \mu,\dot{S_i}(x_i, y_i, p_i) = -S_i + ev_i
\end{equation}

Spatio-temporal surfaces represent a kind of local memory and have been shown to improve the performance of event-based vision processing algorithms because \cite{Lagorce_Orchard_Galluppi_Shi_Benosman_2017,Sironi_Brambilla_Bourdis_Lagorce_Benosman_2018}.

% \subsubsection{Physicality of logarithmic polarity changes}
% Importantly, the polarity changes measured by event cameras have a direct physical interpretation in that they measure the \textit{change} in luminosity in time.

% Event cameras react to changes in brightness separately for each pixel, unlike ordinary cameras, which gather entire pictures at a rate dictated by an external clock \cite{Posch_Retinomorphic}.
% The event-based paradigm is compared against discrete frames in Figure \ref{fig:ebv}.
% They output asynchronous events as precisely timed digital discrete-valued ``spikes'' sequences, representing logarithmic brightness changes at a particular time \cite{Tobi_2016}.
% Compared to conventional frame-based cameras, event-based cameras carry significant advantages, such as higher temporal resolution, less motion blurring, lower latency, higher dynamic range, and less power consumption \cite{Amir_CVPR,Caviar,Jorg_Pencil_Robot}.

\subsection*{Scale-space theory over space and time} \label{sec:scale-space}
\begin{figure}
  \includegraphics[width=\textwidth]{figures/covariance_spatial_temporal.pdf}
  \caption{
    \textbf{Left}: Covariance property for spatial smoothing under spatial affine transformations.
    The order of the affine (horizontal) and Gaussian (vertical) transformations can be interchanged: we obtain the same result when going from the lower left corner to the upper right corner.
    The pathways reflect the two different possible ways of ordering the image transformations.
    \textbf{Right}: Covariance property for temporal scaling.
    Here, a temporal scaling with some factor $S_t$ (horizontal) and temporal smoothing with a causal kernel $h(t;\; \tau)$ (vertical) commute.
    Adapted from \cite{Lindeberg_2023}.
  }
  \label{fig:cov_commute}
\end{figure}

Consider an image $f: \mathbb{R}^2 \to \mathbb{R}$ with a scale-space
representation $L : \mathbb{R}^2 \times \mathbb{R}_+ \to \mathbb{R}$
of the image and a positive scale parameter $s$ (scale-\textit{space} in the formal sense, not the spatial sense \cite{Koenderink_1984}).
At scale $s = 0$, $L$ is defined as the input image
\begin{equation} \label{eq:unit}
  L(\cdot;\; 0) = f(\cdot)
\end{equation}
and at $s > 0$, when the scale is more \textit{coarse}, we define $L$ as the convolution of $f$ and a \textit{scale-space kernel} $g: \mathbb{R}^2 \times \mathbb{R}_+ \to \mathbb{R}$
\begin{equation}
  L(\cdot;\; s) = g(\cdot;\; s) * f
\end{equation}
When $s > 0$, $L$ becomes a ``blurred'' representation of the input image, similar to the blur that would appear through the diffusion of the image RGB values or light intensity \cite{Koenderink_1984}.
To faithfully represent $f$ at scale $s$, we require that $g$ must not
enhance the local extrema, in the sense that the value at local maxima
must not increase, and the values at local minima must not decrease \cite{Lindeberg_2011}.
The canonical choice of such a function is the Gaussian kernel, which
also carries a number of useful properties such as linearity, a semi-group structure, and shift and scale covariance \cite[pp. 38-40]{Lindeberg_2011}
\begin{equation} \label{eq:gaussian}
  g(x;\; \Sigma_s) = \frac{1}{2\pi \sqrt{\text{det}\ \Sigma}}
  e^{-x^T \Sigma^{-1} x/ 2},
\end{equation}
where $\Sigma_s$ is a scale-dependent symmetric positive definite
covariance matrix.

% Consider the domain of 2-dimensional images described as a function $\mathbb{R}^2 \to \mathbb{R}^K$ that maps two coordinates to $K$-channelled real numbers.
% ``Blurring'' the signal in such an image by increasing $s$ corresponds to diffusing the signal with an increasingly large neighboring region \cite{Koenderink_1984}.

% Note that we here are concerned with continuous signals.
% We refer the reader to \cite{Lindeberg_1990} for an in-depth application of scale-space theory for discrete signals.

\subsubsection*{Affine covariance over 2-d image space}
Affine transformations are automorphisms over Euclidean spaces that
can be considered as compositions of translations, scale
transformations, rotations, and shearing operations.
%(defined in the Supplementary Material).

Here, we consider two images $f'(x')$ and $f(x)$ that are related
according to an affine transformation $x' = A \, x$,
such that $f'(x') = f(x)$. Provided that the spatial covariance
matrices $\Sigma'$ and $\Sigma$ in the two domains are related
according to
\begin{equation}
  \label{eq:affine_cov}
  \Sigma' = A\,\Sigma\,A^T
\end{equation}
the corresponding affine scale-space representations $L'$ and $L$ of
$f'$ and $f$ defined by convolution with affine Gaussian kernels
of the form according to equation~(\ref{eq:gaussian}), and with
respective covariance matrices $\Sigma'$ and $\Sigma$, will then be
equal \cite[eq. 16]{Lindeberg_Garding_1994}
\begin{equation}
  \label{eq:affine_scale_spaces}
  L'(x';\; s, \Sigma') = L(x;\; s, \Sigma).
\end{equation}
This covariance property under spatial affine transformations stems from the affine Gaussian kernel in Equation~\eqref{eq:gaussian} being closed regarding affine transformations in the image plane.
This, in turn, implies that convolutions with affine Gaussian kernels can perfectly capture any affine deformations, which is crucial to robustly handle the ``natural image transformations that arise when viewing objects and events in natural environments'' \cite[p. 10]{Lindeberg_2023}.
Figure \ref{fig:cov_commute} (left) illustrates the commutative diagram for spatial covariance for affine transformations under spatial smoothing kernels.

% Signals projected onto a surface 
% The notion of scale-spaces have been particularly successful within computer vision, because it decomposes vision signals in a way that is both intuitive and provably correct.

% Finding ways to recognize patterns and objects in computer vision

\subsubsection*{Scale covariance over time}
Just like \textit{spatial} signals can be parameterized by their scale, so can \textit{temporal} signals be parameterized by the temporal scale, or temporal extent \cite{Koenderink_1988}.
% A ballistic trajectory is an example of a temporal signal where the time scale (velocity) carries tremendous importance.
The principle of temporal causality separates the temporal domain from the spatial domain, which implies that any operation in time should be one-sided, only making use of what has happened \textit{backwards} in time.
Gaussian kernels are symmetric around the origin and, therefore,
impractical to use as temporal kernels in real-time scenarios.
Lindeberg and Fagerstr{\"o}m \cite{Lindeberg_Fagerstrom_1996} explored
this phenomenon and established the truncated exponential kernels as the only primitive scale-space kernels with one-sided support,
assuming that the temporal smoothing process over a 1-dimensional temporal domain must not create new local extrema from finer to coarser levels of temporal scales
\begin{equation} \label{eq:h_exp_2}
  h_{exp}(t, \mu) = \begin{cases}
    \frac{1}{\mu} \, e^{-t/\mu} & t > 0         \\
    0                           & t \leqslant 0
  \end{cases}
\end{equation}
where $\mu$ constitutes the temporal time constant of the temporal
smoothing process.
Using the temporal kernel, we arrive at a temporal multi-channel representation $L$ for some signal $f\colon \mathcal{R} \to \mathcal{R}$ \cite[eq. 14]{Lindeberg_Fagerstrom_1996}:
\begin{equation} \label{eq:temporal_channel_2}
  L(t;\; \mu) = \int_{u=0}^{\infty} f(t - u) \, h_{exp}(u;\; \mu) \, du.
\end{equation}
% Composing a set of such kernels in parallel with varying time
% constants constitutes one way of handling multiple temporal scales.
% This was explored in \cite[eq. 16]{Lindeberg_Fagerstrom_1996} where a number of kernels are composed in parallel with constants $\mu$, where $\mu_k = \sqrt{\tau_k}$ for $k \in K$ number of temporal scale spaces:
% \begin{equation}
%   h_{composed}(\cdot;\; \tau_k) = h_{exp}(\cdot;\; \mu_k)
% \end{equation}
% This leads us to the following temporal scale covariance property
% between two temporally smoothed signals: given 
% $t' = S_t \, t$ and 
% $\tau' = \mu'^2 = S_^2 \tau$% S_t^2 \, \mu^2$
% (further details in the Supplementary Material).
% \begin{equation} \label{eq:temporal_scale_kernel}
% L'(t';\; \tau') = L(t;\; \tau)
% \end{equation}
It is common in the literature to define multiple scales by composing sets of truncated exponential kernels in cascade.
That approach has the property that the number of local extrema in a 1-dimensional smoothed temporal signal is guaranteed to not increase with scale from any finer to any coarser level of scale.
If the multiscale representation is defined by using a single truncated exponential filter for each scale channel, a corresponding simplifying property will only hold between the input signal and the temporally smoothed signal in a specific scale channel, not in relation to arbitrary pairs of scale channels.

Logarithmic distribution of temporal scales ...

\subsection{Dataset}
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/fig_dataset.png}
  \caption{Dataset with superimposed triangles, squares, and circles on a virtual scene, sampled from $p=1.0$ \textbf{(A)} and $p=0.2$ \textbf{(B)}.
    The shapes are transformed by translation (T), scaling (S), rotation (R), and affine (translation, scaling, rotation, and shearing) operations.}
  \label{fig:dataset}
\end{figure}

We simulate an event-based dataset consisting of a virtual background with superimposed shapes.
The virtual background is extracted from the Neurorobotics Platform \cite{Falotico_2017}, and exists purely to provide structured noise.
The shapes in the foreground constitute the real signal.
We use three simple geometries, a triangle, a square, and a circle, that move around the scene according to four different types of transformations: translation, scaling, rotation, and affine (adding shearing).
Each transformation changes over time according to principle of Brownian motion, according to $\dot{x} = -\theta x + \eta(t)$ where $\theta$ controls the rate of change and $\eta$ is a Gaussian noise process.
We concatenate the transformations in sequence to produce four disjoint datasets, shown in Figure \ref{fig:dataset} (top).
We additionally generate datasets where we vary the sparsity of the data by sampling the shape masks from a Bernoulli distribution with varying probability $p \in \{0.01, 0.1, 0.2, 0.4, 0.6, 0.8, 1.0\}$.
Finally, we add 5\textperthousand\, Bernoulli-distributed background noise.
Figure \ref{fig:dataset} (bottom) shows data sampled with $p=0.2$.
It is almost invisible to the human eye against the structured background noise.
More details on the dataset is available in the Supplementary Material.

\subsection{Model and training} \label{sec:model}
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/model.png}
  \caption{
    We use a standard 4-block convolutional neural network architecture in eight variations depending on the number of input channels (1 or 3), and initialization scheme for the spatial and temporal layers.
    As the model output, the green coordinate transform block produces a set of three coordinate-pairs that predicts the position of the three shapes in camera space.
  }
  \label{fig:model_architecture}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/varying_frames.png}
  \caption{Performance of the multi-channel model given varying input frames.}
  \label{fig:varying_frames}
\end{figure}

We use a simple convolutional model architecture with four blocks, shown in Figure \ref{fig:model_architecture} \textbf{(A)}, with interchangeable activation functions.
The first two such functions are the leaky integrator, coupled with a rectified linear unit (ReLU) to induce a (spatial) nonlinearity, and the leaky integrate-and-fire models.
To compare against a baseline, we additionally construct a stateless Single Channel (SC) model using a single rectified linear unit (ReLU) activations instead of the temporal kernels.
We further add one variant of the ReLU model that performs inference on six consecutive frames instead of one, to compensate for the lack of temporal memory, which we refer to as the Multi Channel (MC) model.
The six frames were discovered experimentally by training models with a varying number of frames, shown in Figure~\ref{fig:varying_frames}.
To convert the latent activation space from the fourth block into 2-dimensional coordinates on which we can regress, we apply a differentiable coordinate transformation layer introduced in \cite{Pedersen_2023}.
The method effectively finds the spatial average in two dimensions, as shown in Figure~\ref{fig:varying_frames} \textbf{(C)}.
Note that the coordinate transform uses leaky integrator neurons for both the spiking and non-spiking model architectures.
Each model was trained using backpropagation through time on datasets consists of 4000 movies with 50 frames of 1ms duration, with 20\% of the dataset held for model validation.
The full sets of parameters, along with steps to reproduce the experiments, are available in the Supplementary Material and online at \url{https://github.com/jegp/nrf}.

Each block in the model consists of a spatial convolution, an activation function, a batch normalization layer, and a dropout layer with $10\%$ probability.
The temporal activation functions and the first two spatial convolutional layers are initialized according to theory.
The spatial convolution is parameterized over the number of scales, orientation as well as eccentricity of the covariance matrix of the receptive field, and the number of spatial derivatives.
The first convolutional block uses four spatial scales, derived across the 0th, $\partial_x$, $\partial_y$, and $\partial_{xy}$ derivatives, across a single temporal scale.
The second block uses two spatial scales, three orientations, two eccentricities, and the same directional derivatives as above across four temporal scales.
The convolution in the third block is uniformly initialized, but with four temporal scale-space channels.
All our uniformly initialized parameters follow the uniform distribution $\mathcal{U}(-\sqrt{k}, \sqrt{k})$ where $k = 1 / \sqrt{c_{in}}$ and $c_{in}$ is the number of input channels.
